SummEval: Re-evaluating Summarization Evaluation

The scarcity of comprehensive up-to-date studies on evaluation metrics for text summarization and the lack of consensus regarding evaluation protocols continue to inhibit progress. We address the existing shortcomings of summarization evaluation methods along five dimensions: 1) we re-evaluate 14 automatic evaluation metrics in a comprehensive and consistent fashion using neural summarization model outputs along with expert and crowd-sourced human annotations, 2) we consistently benchmark 23 recent summarization models using the aforementioned automatic evaluation metrics, 3) we assemble the largest collection of summaries generated by models trained on the CNN/DailyMail news dataset and share it in a unified format, 4) we implement and share a toolkit that provides an extensible and unified API for evaluating summarization models across a broad range of automatic metrics, 5) we assemble and share the largest and most diverse, in terms of model types, collection of human judgments of model-generated summaries on the CNN/Daily Mail dataset annotated by both expert judges and crowd-source workers. We hope that this work will help promote a more complete evaluation protocol for text summarization as well as advance research in developing evaluation metrics that better correlate with human judgments.

==> misc.tex <==
% \begin{table*}[h!]\centering
%  \begin{adjustbox}{max width=\textwidth}
%   \begin{tabular}{|c|c|c|c|c|}
%   \hline 
%     \textbf{Metric} & Coherence & Consistency & Fluency & Relevance \\ \hline
% \multicolumn{5}{c}{\textbf{All models}} \\  \hline
%   ROUGE-1/2/3/ &   0.2011/0.1528/0.1635 &  0.1811/0.1583/0.1587 &  0.1496/0.0996/0.0907 &  \textbf{0.3565}/0.2685/0.2611  \\ \hline
%   ROUGE-4/L &   0.1516/0.1564 &  0.1522/0.1578 &  0.0942/0.1382 &  0.2313/0.3347  \\ \hline
%   ROUGE-su*/w &   0.1897/0.1525 &  0.1678/0.1648 &  0.1360/0.1209 &  0.3291/0.3283  \\ \hline
%   ROUGE-we (1/2/3) &   0.202/0.1525/0.127 &  0.1832/0.1319/0.1053 &  0.1513/0.0882/0.0567 &  \textbf{0.3546}/0.2895/0.2634  \\ \hline
%   S3 (pyr/resp) &   0.1667/0.1616 &  0.1624/0.1609 &  0.0813/0.0822 &  \textbf{0.3469}/0.3227  \\ \hline
%   BertScore (p/r/f) &   0.1449/0.1737/0.1854 &  0.1500/0.2082/0.2030 &  0.2056/0.1662/0.2162 &  0.1959/\textbf{0.3503}/0.3192  \\ \hline
%   MoverScore &   0.2115 &  0.1899 &  0.2005 &  0.3114  \\ \hline
%   SMS  & 0.1797 & 0.1794 & 0.1701 & 0.2750 \\ \hline
%   SummaQA\^ & 0.0835 & 0.0802 & -0.0298 & 0.2626 \\ \hline
%  BLEU  & \textbf{0.2212} & 0.1750 & 0.1374 & \textbf{0.3561} \\ \hline
%  CHRF  & 0.2009 & 0.2110 & 0.1716 & 0.2593 \\ \hline
%  CIDEr  & 0.1586 & 0.1832 & 0.1311 & 0.3237 \\ \hline
%  METEOR  & 0.0290 & 0.0336 & 0.0714 & -0.0055 \\ \hline

%   Length\^  & 0.1623 & 0.1655 & 0.1036 & 0.3310 \\ \hline
%   Novel n-gram (1/2/3)\^ &   0.1108/0.003/-0.0655 &  \textbf{-0.3195}/\textbf{-0.4417}/\textbf{-0.466} &  \textbf{-0.2238}/\textbf{-0.3231}/\textbf{-0.3499} &  -0.1043/-0.1701/-0.1959  \\ \hline
%   Repeated n-gram (1/2/3)\^ &   \textbf{-0.2445/-0.3205/-0.2475} &  -0.1309/-0.1539/-0.0801 &  -0.2130/-0.2261/-0.1619 &  -0.0396/-0.1733/-0.1264  \\ \hline
%   Stats (cov/comp/den)\^ &   0.0402/0.0506/\textbf{0.2775} &  \textbf{0.4613}/-0.0604/\textbf{0.2941} &  \textbf{0.3420}/0.0236/\textbf{0.2488} &  0.2026/-0.2020/0.2596  \\ \hline
 
%   \end{tabular}
%   \end{adjustbox}
%   \caption{Pearson correlations of automatic metrics metrics with our expert annotations along four quality dimensions using all 11 available reference summaries. \^{} denotes models which only make use of the source document.}
%   \label{correlations_11}
% \end{table*}








% % % \begin{table*}[h!]\centering
% % %  \begin{adjustbox}{max width=\textwidth}
% % %   \begin{tabular}{|c|c|c|c|c|}
% % %   \hline 
% % %     \textbf{Metric} & Coherence & Consistency & Fluency & Relevance \\ \hline
% % %   ROUGE-1/2/3/ &   0.2011/0.1528/0.1635 &  0.1811/0.1583/0.1587 &  0.1496/0.0996/0.0907 &  \textbf{0.3565}/0.2685/0.2611  \\ \hline
% % %   ROUGE-4/L &   0.1516/0.1564 &  0.1522/0.1578 &  0.0942/0.1382 &  0.2313/0.3347  \\ \hline
% % %   ROUGE-su*/w &   0.1897/0.1525 &  0.1678/0.1648 &  0.1360/0.1209 &  0.3291/0.3283  \\ \hline
% % %   ROUGE-we (1/2/3) &   0.202/0.1525/0.127 &  0.1832/0.1319/0.1053 &  0.1513/0.0882/0.0567 &  \textbf{0.3546}/0.2895/0.2634  \\ \hline
% % %   S3 (pyr/resp) &   0.1667/0.1616 &  0.1624/0.1609 &  0.0813/0.0822 &  \textbf{0.3469}/0.3227  \\ \hline
% % %   BertScore (p/r/f) &   0.1449/0.1737/0.1854 &  0.1500/0.2082/0.2030 &  0.2056/0.1662/0.2162 &  0.1959/\textbf{0.3503}/0.3192  \\ \hline
% % %   MoverScore &   0.2115 &  0.1899 &  0.2005 &  0.3114  \\ \hline
% % %   SMS  & 0.1797 & 0.1794 & 0.1701 & 0.2750 \\ \hline
% % %   SummaQA\^ & 0.0835 & 0.0802 & -0.0298 & 0.2626 \\ \hline
% % %  BLEU  & \textbf{0.2212} & 0.1750 & 0.1374 & \textbf{0.3561} \\ \hline
% % %  CHRF  & 0.2009 & 0.2110 & 0.1716 & 0.2593 \\ \hline
% % %  CIDEr  & 0.1586 & 0.1832 & 0.1311 & 0.3237 \\ \hline
% % %  METEOR  & 0.0290 & 0.0336 & 0.0714 & -0.0055 \\ \hline

% % %   Length\^  & 0.1623 & 0.1655 & 0.1036 & 0.3310 \\ \hline
% % %   Novel n-gram (1/2/3)\^ &   0.1108/0.003/-0.0655 &  \textbf{-0.3195}/\textbf{-0.4417}/\textbf{-0.466} &  \textbf{-0.2238}/\textbf{-0.3231}/\textbf{-0.3499} &  -0.1043/-0.1701/-0.1959  \\ \hline
% % %   Repeated n-gram (1/2/3)\^ &   \textbf{-0.2445/-0.3205/-0.2475} &  -0.1309/-0.1539/-0.0801 &  -0.2130/-0.2261/-0.1619 &  -0.0396/-0.1733/-0.1264  \\ \hline
% % %   Stats (cov/comp/den)\^ &   0.0402/0.0506/\textbf{0.2775} &  \textbf{0.4613}/-0.0604/\textbf{0.2941} &  \textbf{0.3420}/0.0236/\textbf{0.2488} &  0.2026/-0.2020/0.2596  \\ \hline
 
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \caption{Pearson correlations of automatic metrics metrics with our expert annotations along four quality dimensions using all 11 available reference summaries. \^{} denotes models which only make use of the source document.}
% % %   \label{correlations_11}
% % % \end{table*}






% % % \begin{table*}[h!]\centering
% % %  \begin{adjustbox}{max width=\textwidth}
% % %   \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% % %   \hline 
% % %     \textbf{Method} & ROUGE-1/2/3/4/L/su*/w & MoverScore & BertScore & SummaQA & SMS & S3 (pyr/resp) & ROUGE-WE-(1/2/3)   \\ \hline
% % %     M0 - \textbf{LEAD-3} & 0.3994/0.1746/0.0990/0.0647/0.3606/0.1377/0.2072 & 0.1679 & 0.3742 & 0.1652 & 0.1050 & 1.3045/1.4716 & 0.7347/0.7000/0.7419 \\ \hline
% % %     \multicolumn{8}{|c|}{\textit{Extractive Models}} \\ \hline
% % %     M1 - \textbf{NEUSUM} \citep{zhou-etal-2018-neural} & 0.4130/0.1893/0.1109/0.0742/0.3768/0.1495/0.2156 & 0.1839 & 0.3955 & 0.1700 & 0.1062 & 1.3025/1.4678 & 0.7484/0.7073/0.7517  \\ \hline
% % %     M2 - \textbf{BanditSum} \citep{dong-etal-2018-banditsum} & 0.4137/0.1868/0.1086/0.0721/0.3759/0.1513/0.2139 & 0.1815 & 0.3938 & 0.1324 & 0.1058 & 1.2928/1.4451 & 0.7682/0.7217/0.7711  \\ \hline
% % %     M3 - \textbf{LATENT}  \citep{zhang-etal-2018-neural-latent} & 0.4136/0.1867/0.1085/0.0721/0.3757/0.1512/0.2138 & 0.1814 & 0.3936 & 0.1645 & 0.1058 & 1.2928/1.4451 & 0.7681/0.7217/0.7710  \\ \hline
% % %     M4 - \textbf{REFRESH} \citep{narayan-etal-2018-ranking} &  0.3972/0.1807/0.1042/0.0690/0.3621/0.1340/0.2129 & 0.1720 & 0.3903 & 0.1944 & 0.1088 & 1.3534/1.5732 & 0.6568/0.6392/0.6593  \\ \hline
% % %     M5 - \textbf{RNES} \citep{wu2018learning} &  0.4088/0.1878/0.1102/0.0736/0.3719/0.1446/0.2163 & 0.1802 & 0.3997 & 0.1794 & 0.1107 & 1.3343/1.5317 & 0.7047/0.6781/0.7093  \\ \hline
% % %     M6 - \textbf{JECS} \citep{xu-durrett-2019-neural} & 0.4144/0.1846/0.1063/0.0699/0.3760/0.1485/0.2135 & 0.1805 & 0.3925 & 0.1644 & 0.1048 & 1.3014/1.4557 & 0.7651/0.7237/0.7716 \\ \hline
% % %     M7 - \textbf{STRASS} \citep{bouscarrat-etal-2019-strass} & 0.3377/0.1237/0.0650/0.0416/0.2790/0.1052/0.1559 & 0.1079 & 0.3090 & 0.1367 & 0.1023 & 1.2202/1.3303 & 0.7416/0.6944/0.7557 \\ \hline
% % %     \multicolumn{8}{|c|}{\textit{Abstractive Models}} \\ \hline
% % %     M8 - \textbf{Pointer Generator } \citep{see-etal-2017-get} &  0.3921/0.1723/0.1003/0.0674/0.3599/0.1435/0.1999 & 0.1643 & 0.3763 & 0.1398 & 0.0974 & 1.2226/1.3339 & 0.7915/0.7334/0.7990  \\ \hline
% % %     M9 - \textbf{Fast-abs-rl} \citep{chen-bansal-2018-fast} & 0.4057/0.1774/0.0975/0.0616/0.3806/0.1439/0.2112 & 0.1748 & 0.3918 & 0.1431 & 0.0847 & 1.2743/1.4055 & 0.7943/0.7401/0.7998  \\ \hline
% % %     M10 - \textbf{Bottom-Up} \citep{gehrmann-etal-2018-bottom} &  0.4124/0.1870/0.1064/0.0695/0.3815/0.1543/0.2084 & 0.1830 & 0.3964 & 0.1408 & 0.0925 & 1.1783/1.2830 & 0.7979/0.7331/0.8023  \\ \hline
% % %     M11 - \textbf{Improve-abs} \citep{kryscinski-etal-2018-improving} &  0.3985/0.1720/0.0927/0.0567/0.3730/0.1431/0.2073 & 0.1652 & 0.3826 & 0.1341 & 0.0816 & 1.2718/1.4008 & 0.7821/0.7237/0.7819   \\ \hline
% % %     M12 - \textbf{Unified-ext-abs} \citep{hsu-etal-2018-unified} &  0.4038/0.1790/0.1039/0.0695/0.3675/0.1484/0.2074 & 0.1739 & 0.3832 & 0.1530 & 0.1038 & 1.2791/1.4178 & 0.7771/0.7284/0.7827  \\ \hline
% % %     M13 - \textbf{ROUGESal}  \citep{pasunuru-bansal-2018-multi} & 0.4016/0.1797/0.1053/0.0709/0.3679/0.1497/0.2058 & 0.1722 & 0.3837 & 0.1475 & 0.1009 & 1.2438/1.3675 & 0.7878/0.7322/0.7922  \\ \hline
% % %     M14 - \textbf{Multi-task (Ent + QG )} \citep{guo-etal-2018-soft} &  0.3952/0.1758/0.1037/0.0705/0.3625/0.1476/0.2007 & 0.1670 & 0.3759 & 0.1360 & 0.0982 & 1.2049/1.3103 & 0.7973/0.7348/0.8024 \\ \hline
% % %     M15 - \textbf{Closed book decoder} \citep{jiang-bansal-2018-closed} & 0.3976/0.1760/0.1031/0.0696/0.3636/0.1472/0.2033 & 0.1699 & 0.3783 & 0.1456 & 0.1009 & 1.2498/1.3717 & 0.7878/0.7341/0.7950 \\ \hline
% % %     M16 - \textbf{SENECA } \citep{sharma-etal-2019-entity} & 0.4151/0.1836/0.1052/0.0681/0.3806/0.1520/0.2112 & 0.1811 & 0.3907 & 0.1404 & 0.1005 & 1.2357/1.3555 & 0.7985/0.7381/0.8038 \\ \hline
% % %     M17 -  \textbf{T5}  \citep{2019t5} & 0.4479/0.2205/0.1336/0.0920/0.4172/0.1879/0.2291 & 0.2376 & 0.4450 & 0.1437 & 0.1046 & 1.2121/1.3403 & 0.8099/0.7498/0.8183  \\ \hline
% % %     M18 - \textbf{NeuralTD} \citep{bohm-etal-2019-better} &  0.4004/0.1762/0.1000/0.0650/0.3723/0.1452/0.2085 & 0.1697 & 0.3949 & 0.1440 & 0.0916 & 1.2776/1.4146 & 0.7802/0.7229/0.7740  \\ \hline
% % %     M19 - \textbf{BertSum-abs} \citep{liu-lapata-2019-text} & 0.4163/0.1944/0.1156/0.0785/0.3554/0.1625/0.1979 & 0.1894 & 0.3855 & 0.1385 & 0.1071 & 1.1998/1.3165 & 0.7930/0.7361/0.8084  \\ \hline
% % %     M20 - \textbf{GPT-2} \citep{ziegler2019fine} (supervised) & 0.3981/0.1758/0.0993/0.0649/0.3674/0.1470/0.2006 & 0.1750 & 0.3915 & 0.1299 & 0.0930 & 1.1545/1.2519 & 0.7853/0.7181/0.7834   \\ \hline
% % %     M21 - \textbf{UniLM} \citep{dong2019unified} & 0.4306/0.2044/0.1218/0.0824/0.4013/0.1714/0.2228 & 0.2112 & 0.4122 & 0.1455 & 0.0957 & 1.2565/1.3872 & 0.8003/0.7477/0.8131  \\ \hline
% % %     M22 - \textbf{BART} \citep{lewis2019bart} & 0.4416/0.2128/0.1285/0.0880/0.4100/0.1818/0.2266 & 0.2259 & 0.4264 & 0.1457 & 0.1037 & 1.2426/1.3683 & 0.8149/0.7575/0.8295 \\ \hline
% % %     M23 - \textbf{Pegasus} \citep{zhang2019pegasus} (huge news) & 0.4408/0.2147/0.1295/0.0889/0.4103/0.1821/0.2273 & 0.2286 & 0.4377 & 0.1497 & 0.1049 & 1.2397/1.3782 & 0.7982/0.7449/0.8071 \\ \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \caption{Model output scores for each of the metrics available in our toolkit.}
% % %   \label{model_scores_1}
% % % \end{table*}


% % % \begin{table*}[h!]\centering
% % %  \begin{adjustbox}{max width=\textwidth}
% % %   \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% % %   \hline 
% % %     \textbf{Method} &  METEOR & CHRF & BLEU & CIDEr & Length & Stats (cov/comp/den) & Novel(1/2/3) & Repeated (1/2/3) \\ \hline
% % %     M0 - \textbf{LEAD-3}  & 0.2141 & 0.3892 & 11.4270 & 0.0290 & 87.4 & 0.9825/9.6262/57.8001 & 0.1586/0.2701/0.3551 & 0.2086/0.0310/0.0310 \\ \hline
% % %     \multicolumn{9}{|c|}{\textit{Extractive Models}} \\ \hline
% % %     M1 - \textbf{NEUSUM} \citep{zhou-etal-2018-neural} &  0.2183 & 0.3946 & 12.7784 & 0.0403 & 84.4 & 0.9819/9.8047/32.8574 & 0.1758/0.3095/0.4043 & 0.2325/0.0531/0.0531 \\ \hline
% % %     M2 - \textbf{BanditSum} \citep{dong-etal-2018-banditsum} &  0.2124 & 0.3897 & 12.9761 & 0.0481 & 78.5 & 0.9836/10.2810/40.4265 & 0.1750/0.3070/0.4023 & 0.2384/0.0573/0.0573 \\ \hline
% % %     M3 - \textbf{LATENT}  \citep{zhang-etal-2018-neural-latent} &  0.2123 & 0.3897 & 12.9725 & 0.0479 & 78.5 & 0.9834/10.2809/40.4095 & 0.1751/0.3072/0.4025 & 0.2384/0.0573/0.0573 \\ \hline
% % %     M4 - \textbf{REFRESH} \citep{narayan-etal-2018-ranking}  & 0.2395 & 0.4526 & 10.6568 & 0.0241 & 114.6 & 0.9850/7.1059/53.1928 & 0.0149/0.0368/0.0623 & 0.2127/0.0289/0.0289 \\ \hline
% % %     M5 - \textbf{RNES} \citep{wu2018learning} &   0.2300 & 0.4062 & 11.2203 & 0.0230 & 99.9 & 0.9938/7.9032/67.7089 & 0.1564/0.2709/0.3591 & 0.2451/0.0540/0.0540 \\ \hline
% % %     M6 - \textbf{JECS} \citep{xu-durrett-2019-neural} & 0.2122 & 0.4310 & 12.5659 & 0.1184 & 79.8 & 0.9874/10.1111/26.6943 & 0.0140/0.0712/0.1291 & 0.2041/0.0327/0.0327 \\ \hline
% % %     M7 - \textbf{STRASS} \citep{bouscarrat-etal-2019-strass} &  0.1607 & 0.3330 & 7.8330 & 0.0464 & 76.5 & 0.9969/12.7835/59.9498 & 0.1593/0.2823/0.3726 & 0.1864/0.0343/0.0343 \\ \hline
% % %     \multicolumn{9}{|c|}{\textit{Abstractive Models}} \\ \hline
% % %     M8 - \textbf{Pointer Generator} \citep{see-etal-2017-get}  & 0.1860 & 0.3567 & 13.8247 & 0.0866 & 63.5 & 0.9957/13.1940/26.0880 & 0.1552/0.2841/0.3758 & 0.2015/0.0375/0.0375  \\ \hline
% % %     M9 - \textbf{Fast-abs-rl} \citep{chen-bansal-2018-fast} & 0.2014 & 0.3778 & 12.9812 & 0.0664 & 70.9 & 0.9860/11.0141/9.9859 & 0.1730/0.3767/0.5058 & 0.2157/0.0370/0.0370  \\ \hline
% % %     M10 - \textbf{Bottom-Up} \citep{gehrmann-etal-2018-bottom} &  0.1887 & 0.3523 & 15.1293 & 0.1074 & 56.6 & 0.9811/14.7771/12.6181 & 0.1905/0.3851/0.5094 & 0.1856/0.0211/0.0211 \\ \hline
% % %     M11 - \textbf{Improve-abs} \citep{kryscinski-etal-2018-improving} &  0.2005 & 0.3715 & 11.9816 & 0.0541 & 76.0 & 0.9674/10.6043/8.9755 & 0.1952/0.4229/0.5727 & 0.2499/0.0542/0.0542  \\ \hline
% % %     M12 - \textbf{Unified-ext-abs} \citep{hsu-etal-2018-unified} & 0.2017 & 0.3786 & 12.8457 & 0.0589 & 74.5 & 0.9868/10.7510/33.1106 & 0.1611/0.2886/0.3811 & 0.2177/0.0493/0.0493 \\ \hline
% % %     M13 - \textbf{ROUGESal}  \citep{pasunuru-bansal-2018-multi} & 0.1936 & 0.3668 & 13.8882 & 0.0726 & 66.6 & 0.9853/13.0369/25.2893 & 0.1680/0.3090/0.4071 & 0.2102/0.0458/0.0458  \\ \hline
% % %     M14 - \textbf{Multi-task (Ent + QG )} \citep{guo-etal-2018-soft} &   0.1831 & 0.3539 & 14.5276 & 0.0940 & 60.0 & 0.9853/14.1828/22.2296 & 0.1654/0.3080/0.4051 & 0.1985/0.0411/0.0411 \\ \hline
% % %     M15 - \textbf{Closed book decoder} \citep{jiang-bansal-2018-closed} &  0.1925 & 0.3675 & 13.4158 & 0.0736 & 68.3 & 0.9866/12.0588/27.3686 & 0.1607/0.2941/0.3888 & 0.2074/0.0444/0.0444 \\ \hline
% % %     M16 - \textbf{SENECA} \citep{sharma-etal-2019-entity} &  0.1966 & 0.3660 & 13.7676 & 0.0832 & 65.0 & 0.9880/12.3610/16.7640 & 0.1705/0.3502/0.4591 & 0.2146/0.0303/0.0303   \\ \hline
% % %     M17 -  \textbf{T5}  \citep{2019t5} &  0.2140 & 0.3833 & 19.3891 & 0.1453 & 59.5 & 0.9775/14.2002/12.9565 & 0.2023/0.4171/0.5392 & 0.1810/0.0209/0.0209 \\ \hline
% % %     M18 - \textbf{NeuralTD} \citep{bohm-etal-2019-better} &   0.2038 & 0.3783 & 12.9241 & 0.0565 & 74.4 & 0.9830/10.7768/12.4443 & 0.1748/0.3687/0.4922 & 0.2645/0.0901/0.0901 \\ \hline
% % %     M19 - \textbf{BertSum-abs} \citep{liu-lapata-2019-text} &  0.1876 & 0.3649 & 14.9525 & 0.0984 & 60.9 & 0.9517/13.9197/12.3254 & 0.2001/0.3716/0.4831 & 0.1697/0.0156/0.0156 \\ \hline
% % %     M20 - \textbf{GPT-2} \citep{ziegler2019fine} (supervised) &  0.1759 & 0.3678 & 13.9364 & 0.2512 & 51.8 & 0.9791/15.9839/15.4999 & 0.0305/0.1732/0.2932 & 0.1875/0.0362/0.0362  \\ \hline
% % %     M21 - \textbf{UniLM} \citep{dong2019unified} &  0.2084 & 0.4230 & 15.5736 & 0.2183 & 67.2 & 0.9685/11.5672/11.7908 & 0.0398/0.1791/0.3091 & 0.1722/0.0180/0.0180 \\ \hline
% % %     M22 - \textbf{BART} \citep{lewis2019bart} &  0.2105 & 0.4271 & 17.1005 & 0.3310 & 62.3 & 0.9771/12.8811/15.2999 & 0.0301/0.1483/0.2562 & 0.1627/0.0127/0.0127 \\ \hline
% % %     M23 - \textbf{Pegasus} \citep{zhang2019pegasus} (huge news)  & 0.2189 & 0.3912 & 17.8102 & 0.1157 & 66.8 & 0.9814/12.9473/14.9850 & 0.1944/0.3933/0.5113 & 0.1883/0.0251/0.0251   \\ \hline
% % %   \end{tabular}
% % %   \end{adjustbox}
% % %   \caption{Model output scores for each of the metrics available in our toolkit.}
% % %   \label{model_scores_2}
% % % \end{table*}



% % \begin{table*}[h!]\centering
% %  \begin{adjustbox}{max width=\textwidth}
% %   \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% %   \hline 
% %     \textbf{Method} & ROUGE-1/2/3/4/L/su*/w & ROUGE-WE-(1/2/3) & S3 (pyr/resp) & BertScore & MoverScore & SummaQA & SMS    \\ 
% % \hline
% % \multicolumn{8}{|c|}{\textit{Extractive Models}} \\ \hline
% % M0 - \textbf{LEAD-3}  &       0.3994/0.1746/0.0990/0.0647/0.3606/0.1377/0.2072 & 0.4049/0.2260/0.2172 & 0.5395/0.6328 & 0.3742 & 0.1679 & 0.1652 & 0.1050 \\ \hline
% % M1 - \textbf{NEUSUM} \citep{zhou-etal-2018-neural} &       0.4130/0.1893/0.1109/0.0742/0.3768/0.1495/0.2156 & 0.4186/0.2402/0.2310 & 0.5562/0.6509 & 0.3955 & 0.1839 & 0.1700 & 0.1062 \\ \hline
% %  M2 - \textbf{BanditSum} \citep{dong-etal-2018-banditsum} &       0.4137/0.1868/0.1086/0.0721/0.3759/0.1513/0.2139 & 0.4195/0.2385/0.2300 & 0.5339/0.6306 & 0.3938 & 0.1815 & 0.1324 & 0.1058 \\ \hline
% %  M3 - \textbf{LATENT}  \citep{zhang-etal-2018-neural-latent} &       0.4136/0.1867/0.1085/0.0721/0.3757/0.1512/0.2138 & 0.4194/0.2384/0.2299 & 0.5337/0.6305 & 0.3936 & 0.1814 & 0.1645 & 0.1058 \\ \hline
% % M4 - \textbf{REFRESH} \citep{narayan-etal-2018-ranking} &       0.3972/0.1807/0.1042/0.0690/0.3621/0.1340/0.2129 & 0.4023/0.2318/0.2238 & 0.6395/0.7124 & 0.3903 & 0.1720 & 0.1944 & 0.1088 \\ \hline
% %  M5 - \textbf{RNES} \citep{wu2018learning}&        0.4088/0.1878/0.1102/0.0736/0.3719/0.1446/0.2163 & 0.4153/0.2395/0.2317 & 0.6082/0.6894 & 0.3997 & 0.1802 & 0.1794 & 0.1107 \\ \hline
% %  M6 - \textbf{JECS} \citep{xu-durrett-2019-neural} &        0.4144/0.1846/0.1063/0.0699/0.3760/0.1485/0.2135 & 0.4200/0.2371/0.2283 & 0.5337/0.6284 & 0.3925 & 0.1805 & 0.1644 & 0.1048 \\ \hline
% %  M7 - \textbf{STRASS} \citep{bouscarrat-etal-2019-strass} &      0.3377/0.1237/0.0650/0.0416/0.2790/0.1052/0.1559 & 0.3477/0.1757/0.1656 & 0.3632/0.4939 & 0.3090 & 0.1079 & 0.1367 & 0.1023 \\ \hline
% % \multicolumn{8}{|c|}{\textit{Abstractive Models}} \\ \hline
% %   M8 - \textbf{Pointer Generator} \citep{see-etal-2017-get}  &   0.3921/0.1723/0.1003/0.0674/0.3599/0.1435/0.1999 & 0.3990/0.2226/0.2128 & 0.4328/0.5561 & 0.3763 & 0.1643 & 0.1398 & 0.0974 \\ \hline
% %  M9 - \textbf{Fast-abs-rl} \citep{chen-bansal-2018-fast} &      0.4057/0.1774/0.0975/0.0616/0.3806/0.1439/0.2112 & 0.4123/0.2302/0.2184 & 0.4818/0.5865 & 0.3918 & 0.1748 & 0.1431 & 0.0847 \\ \hline
% %  M10 - \textbf{Bottom-Up} \citep{gehrmann-etal-2018-bottom} &        0.4124/0.1870/0.1064/0.0695/0.3815/0.1543/0.2084 & 0.4192/0.2400/0.2313 & 0.4450/0.5655 & 0.3964 & 0.1830 & 0.1408 & 0.0925 \\ \hline
% %  M11 - \textbf{Improve-abs} \citep{kryscinski-etal-2018-improving} &       0.3985/0.1720/0.0927/0.0567/0.3730/0.1431/0.2073 & 0.4045/0.2300/0.2228 & 0.4899/0.5897 & 0.3826 & 0.1652 & 0.1341 & 0.0816 \\ \hline
% %   M12 - \textbf{Unified-ext-abs} \citep{hsu-etal-2018-unified} &       0.4038/0.1790/0.1039/0.0695/0.3675/0.1484/0.2074 & 0.4097/0.2299/0.2204 & 0.4936/0.5995 & 0.3832 & 0.1739 & 0.1530 & 0.1038 \\ \hline
% %   M13 - \textbf{ROUGESal}  \citep{pasunuru-bansal-2018-multi} &       0.4016/0.1797/0.1053/0.0709/0.3679/0.1497/0.2058 & 0.4078/0.2294/0.2190 & 0.4643/0.5799 & 0.3837 & 0.1722 & 0.1475 & 0.1009 \\ \hline
% %  M14 - \textbf{Multi-task (Ent + QG )} \citep{guo-etal-2018-soft}  &      0.3952/0.1758/0.1037/0.0705/0.3625/0.1476/0.2007 & 0.4015/0.2253/0.2149 & 0.4246/0.5513 & 0.3759 & 0.1670 & 0.1360 & 0.0982 \\ \hline
% %   M15 - \textbf{Closed book decoder} \citep{jiang-bansal-2018-closed} &     0.3976/0.1760/0.1031/0.0696/0.3636/0.1472/0.2033 & 0.4039/0.2263/0.2160 & 0.4591/0.5757 & 0.3783 & 0.1699 & 0.1456 & 0.1009 \\ \hline
% %  M16 - \textbf{SENECA} \citep{sharma-etal-2019-entity}  &       0.4151/0.1836/0.1052/0.0681/0.3806/0.1520/0.2112 & 0.4211/0.2369/0.2282 & 0.4735/0.5836 & 0.3907 & 0.1811 & 0.1404 & 0.1005 \\ \hline
% %  M17 -  \textbf{T5}  \citep{2019t5} &  0.4479/0.2205/0.1336/0.0920/0.4172/0.1879/0.2291 & 0.4543/0.2723/0.2631 & 0.5168/0.6294 & 0.4450 & 0.2376 & 0.1437 & 0.1046 \\ \hline
% % M18 - \textbf{NeuralTD} \citep{bohm-etal-2019-better} &     0.4004/0.1762/0.1000/0.0650/0.3723/0.1452/0.2085 & 0.4063/0.2277/0.2187 & 0.4946/0.5975 & 0.3949 & 0.1697 & 0.1440 & 0.0916 \\ \hline
% % M19 - \textbf{BertSum-abs} \citep{liu-lapata-2019-text} &     0.4163/0.1944/0.1156/0.0785/0.3554/0.1625/0.1979 & 0.4230/0.2454/0.2351 & 0.4664/0.5855 & 0.3855 & 0.1894 & 0.1385 & 0.1071 \\ \hline
% % M20 - \textbf{GPT-2} \citep{ziegler2019fine} (supervised) &        0.3981/0.1758/0.0993/0.0649/0.3674/0.1470/0.2006 & 0.4048/0.2268/0.2170 & 0.4069/0.5373 & 0.3915 & 0.1750 & 0.1299 & 0.0930 \\ \hline
% %  M21 - \textbf{UniLM} \citep{dong2019unified} &      0.4306/0.2044/0.1218/0.0824/0.4013/0.1714/0.2228 & 0.4369/0.2567/0.2483 & 0.5143/0.6210 & 0.4122 & 0.2112 & 0.1455 & 0.0957 \\ \hline
% % M22 - \textbf{BART} \citep{lewis2019bart} &        0.4416/0.2128/0.1285/0.0880/0.4100/0.1818/0.2266 & 0.4472/0.2646/0.2556 & 0.5116/0.6215 & 0.4264 & 0.2259 & 0.1457 & 0.1037 \\ \hline
% % M23 - \textbf{Pegasus} \citep{zhang2019pegasus} (huge news) &       0.4408/0.2147/0.1295/0.0889/0.4103/0.1821/0.2273 & 0.4473/0.2663/0.2568 & 0.5295/0.6372 & 0.4377 & 0.2286 & 0.1497 & 0.1049 \\ \hline
% %   \end{tabular}
% %   \end{adjustbox}
% %   \caption{Model output scores for each of the metrics available in our toolkit.}
% %   \label{model_scores_1}
% % \end{table*}



% \begin{table*}[h!]\centering
%  \begin{adjustbox}{max width=\textwidth}
%   \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%   \hline 
% \textbf{Method} &  BLEU & CHRF & CIDEr & CHRF & Length & Stats (cov/comp/den) & Repeated (1/2/3) \\ \hline
%     \multicolumn{8}{|c|}{\textit{Extractive Models}} \\ \hline
% M0 - \textbf{LEAD-3} &       11.4270 & 0.3892 & 0.2125 & 0.2141 & 87.4475 & 0.9825/9.6262/57.8001 & 0.2086/0.0310/0.0310 \\ \hline
% M1 - \textbf{NEUSUM} \citep{zhou-etal-2018-neural} &       12.7784 & 0.3946 & 0.2832 & 0.2183 & 84.4075 & 0.9819/9.8047/32.8574 & 0.2325/0.0531/0.0531 \\ \hline
% M2 - \textbf{BanditSum} \citep{dong-etal-2018-banditsum} &       12.9761 & 0.3897 & 0.3305 & 0.2124 & 78.5279 & 0.9836/10.2810/40.4265 & 0.2384/0.0573/0.0573 \\ \hline
% M3 - \textbf{LATENT}  \citep{zhang-etal-2018-neural-latent} &       12.9725 & 0.3897 & 0.3305 & 0.2123 & 78.5279 & 0.9834/10.2809/40.4095 & 0.2384/0.0573/0.0573 \\ \hline
%  M4 - \textbf{REFRESH} \citep{narayan-etal-2018-ranking}  &       10.6568 & 0.4526 & 0.0677 & 0.2395 & 114.5684 & 0.9850/7.1059/53.1928 & 0.2127/0.0289/0.0289 \\ \hline
% M5 - \textbf{RNES} \citep{wu2018learning} &        11.2203 & 0.4062 & 0.1559 & 0.2300 & 99.9199 & 0.9938/7.9032/67.7089 & 0.2451/0.0540/0.0540 \\ \hline
% M6 - \textbf{JECS} \citep{xu-durrett-2019-neural} &        12.5659 & 0.4310 & 0.3090 & 0.2122 & 79.7797 & 0.9874/10.1111/26.6943 & 0.2041/0.0327/0.0327 \\ \hline
% M7 - \textbf{STRASS} \citep{bouscarrat-etal-2019-strass}  &      7.8330 & 0.3330 & 0.2945 & 0.1607 & 76.4859 & 0.9969/12.7835/59.9498 & 0.1864/0.0343/0.0343 \\ \hline
% \multicolumn{8}{|c|}{\textit{Abstractive Models}} \\ \hline
%  M8 - \textbf{Pointer Generator } \citep{see-etal-2017-get}  &   13.8247 & 0.3567 & 0.5065 & 0.1860 & 63.5211 & 0.9957/13.1940/26.0880 & 0.2015/0.0375/0.0375 \\ \hline
% M9 - \textbf{Fast-abs-rl} \citep{chen-bansal-2018-fast} &      12.9812 & 0.3778 & 0.4329 & 0.2014 & 70.8600 & 0.9860/11.0141/9.9859 & 0.2157/0.0370/0.0370 \\ \hline
% M10 - \textbf{Bottom-Up} \citep{gehrmann-etal-2018-bottom} &        15.1293 & 0.3523 & 0.6176 & 0.1887 & 56.5715 & 0.9811/14.7771/12.6181 & 0.1856/0.0211/0.0211 \\ \hline
% M11 - \textbf{Improve-abs} \citep{kryscinski-etal-2018-improving} &       11.9816 & 0.3715 & 0.3356 & 0.2005 & 75.9512 & 0.9674/10.6043/8.9755 & 0.2499/0.0542/0.0542 \\ \hline
% M12 - \textbf{Unified-ext-abs} \citep{hsu-etal-2018-unified} &       12.8457 & 0.3786 & 0.3851 & 0.2017 & 74.4663 & 0.9868/10.7510/33.1106 & 0.2177/0.0493/0.0493 \\ \hline
% M13 - \textbf{ROUGESal}  \citep{pasunuru-bansal-2018-multi} &       13.8882 & 0.3668 & 0.4746 & 0.1936 & 66.5575 & 0.9853/13.0369/25.2893 & 0.2102/0.0458/0.0458 \\ \hline
% M14 - \textbf{Multi-task (Ent + QG )} \citep{guo-etal-2018-soft} &      14.5276 & 0.3539 & 0.5749 & 0.1831 & 60.0294 & 0.9853/14.1828/22.2296 & 0.1985/0.0411/0.0411 \\ \hline
%   M15 - \textbf{Closed book decoder} \citep{jiang-bansal-2018-closed} &     13.4158 & 0.3675 & 0.4648 & 0.1925 & 68.2858 & 0.9866/12.0588/27.3686 & 0.2074/0.0444/0.0444 \\ \hline
%   M16 - \textbf{SENECA } \citep{sharma-etal-2019-entity}  &       13.7676 & 0.3660 & 0.5233 & 0.1966 & 64.9710 & 0.9880/12.3610/16.7640 & 0.2146/0.0303/0.0303 \\ \hline
%   M17 -  \textbf{T5}  \citep{2019t5} &  19.3891 & 0.3833 & 0.7763 & 0.2140 & 59.5288 & 0.9775/14.2002/12.9565 & 0.1810/0.0209/0.0209 \\ \hline
%   M18 - \textbf{NeuralTD} \citep{bohm-etal-2019-better}&     12.9241 & 0.3783 & 0.3543 & 0.2038 & 74.4033 & 0.9830/10.7768/12.4443 & 0.2645/0.0901/0.0901 \\ \hline
%   M19 - \textbf{BertSum-abs} \citep{liu-lapata-2019-text} &     14.9525 & 0.3649 & 0.6240 & 0.1876 & 60.8893 & 0.9517/13.9197/12.3254 & 0.1697/0.0156/0.0156 \\ \hline
%      M20 - \textbf{GPT-2} \citep{ziegler2019fine} (supervised) &        13.9364 & 0.3678 & 0.5787 & 0.1759 & 51.8352 & 0.9791/15.9839/15.4999 & 0.1875/0.0362/0.0362 \\ \hline
% M21 - \textbf{UniLM} \citep{dong2019unified} &      15.5736 & 0.4230 & 0.5294 & 0.2084 & 67.1960 & 0.9685/11.5672/11.7908 & 0.1722/0.0180/0.0180 \\ \hline
%  M22 - \textbf{BART} \citep{lewis2019bart} &        17.1005 & 0.4271 & 0.7573 & 0.2105 & 62.2989 & 0.9771/12.8811/15.2999 & 0.1627/0.0127/0.0127 \\ \hline
% M23 - \textbf{Pegasus} \citep{zhang2019pegasus} (huge news) &       17.8102 & 0.3912 & 0.6595 & 0.2189 & 66.7559 & 0.9814/12.9473/14.9850 & 0.1883/0.0251/0.0251 \\ \hline
%   \end{tabular}
%   \end{adjustbox}
%   \caption{Model output scores for each of the metrics available in our toolkit.}
%   \label{model_scores_2}
% \end{table*}

